GRACE: A Granular Benchmark for Evaluating Model Calibration against Human Calibration

Language models are often miscalibrated, leading to confidently incorrect answers. We introduce GRACE, a benchmark for language model calibration that incorporates comparison with human calibration. GRACE consists of question-answer pairs, in which each question contains a series of clues that gradually become easier, all leading to the same answer; models must answer correctly as early as possible as the clues are revealed. This setting permits granular measurement of model calibration based on how early, accurately, and confidently a model answers. After collecting these questions, we host live human vs. model competitions to gather 1,749 data points on human and model teams' timing, accuracy, and confidence. We propose a metric, CalScore, that uses GRACE to analyze model calibration errors and identify types of model miscalibration that differ from human behavior. We find that although humans are less accurate than models, humans are generally better calibrated. Since state-of-the-art models struggle on GRACE, it effectively evaluates progress on improving model calibration.

==> 2025_acl_advcal/sections/90-advcal-tournament.tex <==
% \jbgcomment{Before we move on to our new metric, I think it would be worthwhile to have an analysis that looks more like ECE to get a more straightforward estimate of human calibration.  I think it would go something like:

% - Let's assume that all agents have some internal notion of confidence
% - They have a threshold, and whenever they are over that threshold, they buzz
% - We don't know that for humans, but we do for computers
% - However, we can can plot human ECE error for the ``buzzing'' bin based on where the threshold is (and you can assume that the confidence in uniformly distributed within the bin for humans).  And then compare that calibration error vs. computer models.
% - You can then compute an accuracy \emph{conditioned on the decision to buzz} and we can show the distribution over humans and models

% Then, based on this initial analysis, we can move on to why this falls short of what we want in a metric.

% }

% \efcomment{Just to keep our terminology consistent throughout the paper:

% A buzzpoint is the point within a question at which a human team buzzed.

% A match is a single game between two teams, played on one 20-question packet.

% A round consists of all matches played on one packet (all matches played at the same time).
% }

%\jbgcomment{Survey should also be described here.}




%Prizes were awarded to the top human teams at each tournament. %The primary objectives of the tournament were twofold: to assess whether models could outperform humans when leveraging calibrated confidence and to 
%
% \begin{enumerate}
%     \item They validated that the questions are answerable by humans and provided an extra check on dataset quality.
%     \item They allow us to provide statistics on human performance, including that of humans with varying skill levels, for our dataset. Our dataset thus provides human buzzpoints for future research on calibration measurement.
%     \item They allow us to compare the confidence calibration of humans and models on the same dataset.
% \end{enumerate}

%
%\subsection{Human vs. model matches}


% In the next two sections, we discuss how these buzzpoints are used to ground model calibration in human performance and analyze differences in human and model performance.






==> 2025_acl_advcal/sections/calibrated-examples.tex <==
% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lllll}
% \toprule
% Category & Question & Answer & \metric{} & Model \\ \midrule
% Other Fine Arts & 
% \begin{tabular}{l}
% Three Sea Captains and Garden of Daisies are works from this country. A dance form from this country\\often requires dancers to wear large curly wigs. In a show from this country, "Little Spirit"\\awakens dancers including a goddess and a titular lord. " The book" contains 30 canonical group\\dances from this country. Dancers' legs flail about while their torsos remain still in a dance from\\this country. Feis and oireachtas show a dance from this country, which Michael Flatley popularized\\in the show Riverdance. For 10 points, reels and jigs may be step-danced to songs like "The Rocky\\Road to Dublin" in what country?
% \end{tabular}
% & Ireland & 0.1298 & GPT-4 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Examples}
% \label{tab:example}
% \end{table*}

\section{Calibrated and Miscalibrated Statistics}
We analyze the top 5 calibrated and miscalibrated questions for the six models based on \metric{}. Table~\ref{tab:calibrated-stats} shows the statistics per category.

\begin{table}[t]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Category}} & \multicolumn{2}{c}{\textbf{Miscalibrated}} & \multicolumn{2}{c}{\textbf{Calibrated}} \\ \cmidrule(l){2-5} 
 & \textbf{Verbalized} & \textbf{Logit} & \textbf{Verbalized} & \textbf{Logit} \\ \midrule
American Hist & 0 & 0 & 6.67\% & 3.33\% \\
Biology & 20.0\% & 0 & 20.0\% & 26.67\% \\
Chemistry & 0 & 0 & 0 & 6.67\% \\
Classical Music & 0 & 20.0\% & 10.0\% & 6.67\% \\
Euro Lit & 20.0\% & 0 & 6.67\% & 0 \\
Geo/CE & 20.0\% & 20.0\% & 6.67\% & 10.0\% \\
Geo/CE/other & 0 & 0 & 13.33\% & 6.67\% \\
Other Arts & 0 & 0 & 6.67\% & 6.67\% \\
Other Hist & 0 & 0 & 0 & 3.33\% \\
Painting/Sculpture & 0 & 0 & 3.33\% & 3.33\% \\
Philosophy & 0 & 0 & 6.67\% & 6.67\% \\
Physics & 20.0\% & 0 & 13.33\% & 13.33\% \\
Religion & 20.0\% & 40.0\% & 6.67\% & 3.33\% \\
Social Science & 0 & 0 & 0 & 3.33\% \\
World Hist & 0 & 20.0\% & 0 & 0 \\ \bottomrule
\end{tabular}
}
\caption{Calibrated and miscalibrated analysis based on categories.}
\label{tab:calibrated-stats}
\end{table}

% Hope: put the example here and just in case we need it in the future
